Interactive Answer Set Programming - Preliminary Report

Traditional Answer Set Programming (ASP) rests upon one-shot solving. A logic program is fed into an ASP system and its stable models are computed. The high practical relevance of dynamic applications led to the development of multi-shot solving systems. An operative system solves continuously changing logic programs. Although this was primarily aiming at dynamic applications in assisted living, robotics, or stream reasoning, where solvers interact with an environment, it also opened up the opportunity of interactive ASP, where a solver interacts with a user. We begin with a formal characterization of interactive ASP in terms of states and operations on them. In turn, we describe the interactive ASP shell aspic along with its basic functionalities.

==> background.tex <==

% \section{Background}
% \label{sec:background}

The \clingo~4 series goes beyond its predecessors by providing control capacities
that can be used either through scripting inlets in ASP encodings or corresponding APIs
in Lua and Python.
%
% To this end,
% \clingo~4 provides two declarations.
% First, the \texttt{\#external} declaration allows for defining atoms whose truth value is determined externally,
% either via the aforementioned control capacities or by later addition of defining rules.
% Second, the \texttt{\#program} declaration allows for regrouping rules in subprograms.
%
Details can be found in~\cite{gekakasc14b}.

Similarly we refer the reader to the literature for an introduction to ASP~\cite{gelkah14a,gekakasc12a} and the input language of \clingo~4~\cite{PotasscoUserGuide}.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

